DualFair: Fair Representation Learning at Both Group and Individual Levels via Contrastive Self-supervision

Algorithmic fairness has become an important machine learning problem, especially for mission-critical Web applications. This work presents a self-supervised model, called DualFair, that can debias sensitive attributes like gender and race from learned representations. Unlike existing models that target a single type of fairness, our model jointly optimizes for two fairness criteria - group fairness and counterfactual fairness - and hence makes fairer predictions at both the group and individual levels. Our model uses contrastive loss to generate embeddings that are indistinguishable for each protected group, while forcing the embeddings of counterfactual pairs to be similar. It then uses a self-knowledge distillation method to maintain the quality of representation for the downstream tasks. Extensive analysis over multiple datasets confirms the model's validity and further shows the synergy of jointly addressing two fairness criteria, suggesting the model's potential value in fair intelligent Web applications.

==> section/algo.tex <==

% \normalem
\begin{algorithm}[t!]
\small{
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Indmm \Indmm
\Input{Backbone network $f$, projection head $g$, two prediction heads $h_1$, $h_2$, sample generator $q_\phi$ and $p_\theta$, and the training set $\mathcal{D}$}
\Output{Trained backbone network $f$}
\Indpp \Indpp
\ForEach{batch $\mathcal{B}^s \subset \mathcal{D}$}
{
    $L_{\text{fair-CL}}, L_{\text{self-KD}} \gets 0, 0 $ \\
    $\mathcal{B}^{s}_{\text{pert}} \gets \text{TabMix}(\mathcal{B}^s, \text{Sample}(\mathcal{D} \setminus \mathcal{B}^s))$  \tcp{(Eq.~\ref{eq:tabmix})}
    $\mathcal{B}^{s'}_{\text{cnt}} \gets \text{Convert}(\mathcal{B}^s, q_\phi, p_\theta)$ \tcp{(Sec. 3.2)}
    \ForEach{$\mathbf{x}^s \in \mathcal{B}_s$, $\mathbf{x}^s_{\text{pert}} \in \mathcal{B}^{s}_{\text{pert}}$, and $\mathbf{x}^{s'}_{\text{cnt}} \in \mathcal{B}^{s'}_{\text{cnt}}$}
    {   
        $\mathcal{X}^s_{-} = \{ \mathbf{x} | \mathbf{x} \in \mathcal{B}_s\setminus\{\mathbf{x}^s\} \}$ \\
         \tcp{Fairness-aware contrastive loss (Eq.~\ref{eq:contrast_loss})}
         $L_{\text{fair-CL}} \gets L_{\text{fair-CL}} + L_{\text{gen-c}} (\mathbf{x}^s, \mathbf{x}^{s'}_{\text{cnt}}, \mathcal{X}^s_{-})$ \\ \vspace{2mm}
         \tcp{Self-knowledge distillation loss (Eq.~\ref{eq:self-kd})}
         $\mathbf{p}_{\text{student}} \gets h_2 \circ g \circ f(\mathbf{x}^s_{\text{pert}})$ \\
         $\mathbf{z}_{\text{teacher}} \gets (g \circ f(\mathbf{x}^s)).\text{detach()}$ \\
         $L_{\text{self-KD}} \gets L_{\text{self-KD}} - ({\mathbf{p}_{\text{student}} \over || \mathbf{p}_{\text{student}} ||_2} \cdot {\mathbf{z}_{\text{teacher}}  \over || \mathbf{z}_{\text{teacher}} ||_2})$  \\
    }
    $L_{\text{total}} = {1 \over |\mathcal{B}_s|}(L_{\text{fair-CL}} +  L_{\text{self-KD}})$  \\
    Update weights via back-propagation
}
\caption{Overall training procedure (for one epoch)}}
\label{algo:algorithm}
\end{algorithm}
% \ULforem
